Cooperating Graph Neural Networks with Deep Reinforcement Learning for Vaccine Prioritization

This study explores the vaccine prioritization strategy to reduce the overall burden of the pandemic when the supply is limited. Existing methods conduct macro-level or simplified micro-level vaccine distribution by assuming the homogeneous behavior within subgroup populations and lacking mobility dynamics integration. Directly applying these models for micro-level vaccine allocation leads to sub-optimal solutions due to the lack of behavioral-related details. To address the issue, we first incorporate the mobility heterogeneity in disease dynamics modeling and mimic the disease evolution process using a Trans-vaccine-SEIR model. Then we develop a novel deep reinforcement learning to seek the optimal vaccine allocation strategy for the high-degree spatial-temporal disease evolution system. The graph neural network is used to effectively capture the structural properties of the mobility contact network and extract the dynamic disease features. In our evaluation, the proposed framework reduces 7% - 10% of infections and deaths than the baseline strategies. Extensive evaluation shows that the proposed framework is robust to seek the optimal vaccine allocation with diverse mobility patterns in the micro-level disease evolution system. In particular, we find the optimal vaccine allocation strategy in the transit usage restriction scenario is significantly more effective than restricting cross-zone mobility for the top 10% age-based and income-based zones. These results provide valuable insights for areas with limited vaccines and low logistic efficacy.

==> Src/0.abstract.nan.tex <==
Given a limited vaccine supply, what is the optimal strategy to distribute vaccine that can reduce the total burden over the populations?
Prior works only consider macro-level vaccine distribution strategy for group-level populations that are sub-optimal for subgroup-level population, since xxx. 
%
Therefore, we propose a disease diffusion process (DDP) that simulates the process of disease spreading over time and location. Our DDP can be more accurate for predicting the spread of disease over population and locations through time and thus offer a strong heuristics for determining  the vaccine supply for that subgroup of population and location. 
%
To determine the parameters involved in the DDP model, we use a graph neural network (GNN) to represent the DDP model, where the node in the GNN is xxx and edges is xxx. We then use reinforcement learning algorithm to directly learn the vaccine supply strategy, where the states are the sub-group population and the actions are the number of vaccine supply. In experiment, our DDP model reduces $\ge 7\%$ of infections and deaths than the baseline strategies.
Extensive evaluation shows that the proposed framework is robust to seek the optimal vaccine allocation with diverse mobility patterns in the micro-level disease evolution system.  
In particular, we find the optimal vaccine allocation strategy in the transit usage restriction scenario is significantly more effective than restricting cross-zone mobility for the top 10\% age-based and income-based zones.




